Top-N Recommendation Algorithms: A Quest for the State-of-the-Art

Research on recommender systems algorithms, like other areas of applied machine learning, is largely dominated by efforts to improve the state-of-the-art, typically in terms of accuracy measures. Several recent research works however indicate that the reported improvements over the years sometimes "don't add up", and that methods that were published several years ago often outperform the latest models when evaluated independently. Different factors contribute to this phenomenon, including that some researchers probably often only fine-tune their own models but not the baselines. In this paper, we report the outcomes of an in-depth, systematic, and reproducible comparison of ten collaborative filtering algorithms - covering both traditional and neural models - on several common performance measures on three datasets which are frequently used for evaluation in the recent literature. Our results show that there is no consistent winner across datasets and metrics for the examined top-n recommendation task. Moreover, we find that for none of the accuracy measurements any of the considered neural models led to the best performance. Regarding the performance ranking of algorithms across the measurements, we found that linear models, nearest-neighbor methods, and traditional matrix factorization consistently perform well for the evaluated modest-sized, but commonly-used datasets. Our work shall therefore serve as a guideline for researchers regarding existing baselines to consider in future performance comparisons. Moreover, by providing a set of fine-tuned baseline models for different datasets, we hope that our work helps to establish a common understanding of the state-of-the-art for top-n recommendation tasks.

==> sections/discussion.tex <==
\begin{comment}
TODO, based on results, ideas.
\begin{itemize}
  \item No clear winner
  \item X and Y of take leading positions
  \item Neural methods generally not winning. confirms earlier research \cite{Ferraridacrema2020troubling},\cite{ncfvsmf2020},
  \item NeuMF works well in Sun et al.~for Epinions. This is not the case in our experiment. Are there differences after preprocessing?
  \item larger datasets. maybe beneficial for neural methods, \ref{SteckNetflixAIMagazine,JannachdeSouzaetal2020}
  \item insights regarding beyond-accuracy results?
\end{itemize}

\end{comment}

\begin{comment}
TODO: Create Borda count ranking across datasets and metrics. Discuss it. Mention that we have to be careful what to conclude from such a ranking.

\input{tables/algorithm_ranking} 

\end{comment}

==> sections/related.tex <==
DJ: Probably we don't have a related work section. Unless there are other related comparisons

==> tables/amazon_accuracy.tex <==
\begin{table}[H]
\centering
\caption{Accuracy Results for Amazon Digital Music. The Tables are sorted by nDCG in descending order. The notation \emph{@N} indicates that the metrics are computed considering recommendation lists of \emph{N} elements.}
\label{tab:amazon_accuracy}
%\rowcolors{1}{white}{gray!15}
% \renewcommand{\arraystretch}{0.8}
% \rowcolors{2}{gray!15}{white}
% \begin{tabular}{lrrrrrrrrrrr}\hline
%     \multirow{2}{*}{\textbf{Algorithm}} &\multicolumn{5}{c}{\textbf{Top@10}}&\multicolumn{5}{c}{\textbf{Top@50}} \\
%     \cmidrule(lr){2-6} \cmidrule(l){7-11}
% &\textbf{nDCG} &\textbf{MAP} &\textbf{MRR} &\textbf{Pre} &\textbf{Rec}
% &\textbf{nDCG} &\textbf{MAP} &\textbf{MRR} &\textbf{Pre} &\textbf{Rec}\\\midrule
% MultiVAE &0.054 &0.023 &0.062 &0.016 &0.077 &0.075 &0.012 &0.069 &\underline{0.007} &0.157 \\
% NeuMF &0.056 &0.024 &0.068 &0.015 &0.074 &0.073 &0.012 &0.073 &0.006 &0.136 \\
% \pbeta &\textbf{0.085} &\textbf{0.040} &\textbf{0.115} &\textbf{0.023} &\textbf{0.104} &\textbf{0.106} &\textbf{0.018} &\textbf{0.121} &\textbf{0.008} &0.179 \\
% \easer &0.078 &0.034 &0.100 &0.021 &\underline{0.101} &0.100 &0.016 &0.105 &\textbf{0.008} &0.181 \\
% \slim &\underline{0.081} &\underline{0.037} &\underline{0.106} &\underline{0.022} &\textbf{0.104} &\underline{0.103} &\underline{0.017} &\underline{0.111} &\textbf{0.008} &\underline{0.183} \\
% \ials &0.073 &0.032 &0.093 &0.021 &0.099 &0.097 &0.016 &0.099 &\textbf{0.008} &\textbf{0.185} \\
% BPRMF &0.020 &0.008 &0.023 &0.007 &0.031 &0.032 &0.005 &0.027 &0.003 &0.076 \\
% MF2020 &0.057 &0.024 &0.067 &0.017 &0.083 &0.081 &0.013 &0.074 &\underline{0.007} &0.173 \\
% \userknn &0.081 &\underline{0.037} &0.105 &\underline{0.022} &\textbf{0.104} &0.102 &\underline{0.017} &0.110 &\textbf{0.008} &0.181 \\
% \itemknn &0.071 &0.033 &0.095 &0.018 &0.085 &0.088 &0.015 &0.100 &\underline{0.007} &0.148 \\
% MostPop &0.012 &0.005 &0.016 &0.004 &0.016 &0.019 &0.003 &0.018 &0.002 &0.046 \\
% Random &0.000 &0.000 &0.000 &0.000 &0.001 &0.001 &0.000 &0.001 &0.000 &0.004 \\
% \bottomrule
% \end{tabular}
\scriptsize
\begin{tabularx}{\textwidth}{Xrrrrrr}\toprule
\textbf{Algorithm} &\textbf{nDCG@10} &\textbf{MAP@10} &\textbf{MRR@10} &\textbf{Pre@10} &\textbf{Rec@10} \\\midrule
\pbeta &0.085 &0.040 &0.115 &0.023 &0.104 \\
\slim &0.081 &0.037 &0.106 &0.022 &0.104 \\
\userknn &0.081 &0.037 &0.105 &0.022 &0.104 \\
\easer &0.078 &0.034 &0.100 &0.021 &0.101 \\
\ials &0.073 &0.032 &0.093 &0.021 &0.099 \\
\itemknn &0.071 &0.033 &0.095 &0.018 &0.085 \\
MF2020 &0.057 &0.024 &0.067 &0.017 &0.083 \\
NeuMF &0.056 &0.024 &0.068 &0.015 &0.074 \\
MultiVAE &0.054 &0.023 &0.062 &0.016 &0.077 \\
BPRMF &0.020 &0.008 &0.023 &0.007 &0.031 \\
MostPop &0.012 &0.005 &0.016 &0.004 &0.016 \\
Random &0.000 &0.000 &0.000 &0.000 &0.001 \\
\bottomrule
\end{tabularx}

% \rowcolors{1}{white}{gray!15}
\begin{tabularx}{\textwidth}{Xrrrrrr}\toprule
\textbf{Algorithm} &\textbf{nDCG@20} &\textbf{MAP@20} &\textbf{MRR@20} &\textbf{Pre@20} &\textbf{Rec@20} \\\midrule 
\pbeta &0.094 &0.029 &0.118 &0.015 &0.132 \\
\slim &0.090 &0.027 &0.109 &0.014 &0.134 \\
\userknn &0.090 &0.027 &0.108 &0.014 &0.133 \\
\easer &0.087 &0.026 &0.103 &0.014 &0.131 \\
\ials &0.084 &0.025 &0.096 &0.014 &0.132 \\
\itemknn &0.078 &0.023 &0.098 &0.012 &0.108 \\
MF2020 &0.067 &0.019 &0.071 &0.012 &0.116 \\
NeuMF &0.063 &0.018 &0.071 &0.010 &0.096 \\
MultiVAE &0.062 &0.017 &0.066 &0.011 &0.105 \\
BPRMF &0.025 &0.007 &0.025 &0.005 &0.047 \\
MostPop &0.014 &0.004 &0.017 &0.003 &0.025 \\
Random &0.001 &0.000 &0.001 &0.000 &0.001 \\
\bottomrule
\end{tabularx}

% \rowcolors{1}{white}{gray!15}
\begin{tabularx}{\textwidth}{Xrrrrrr}\toprule
\textbf{Algorithm} &\textbf{nDCG@50} &\textbf{MAP@50} &\textbf{MRR@50} &\textbf{Pre@50} &\textbf{Rec@50} \\\midrule 
\pbeta &0.106 &0.018 &0.121 &0.008 &0.179 \\
\slim &0.103 &0.017 &0.111 &0.008 &0.183 \\
\userknn &0.102 &0.017 &0.110 &0.008 &0.181 \\
\easer &0.100 &0.016 &0.105 &0.008 &0.181 \\
\ials &0.097 &0.016 &0.099 &0.008 &0.185 \\
\itemknn &0.088 &0.015 &0.100 &0.007 &0.148 \\
MF2020 &0.081 &0.013 &0.074 &0.007 &0.173 \\
NeuMF &0.073 &0.012 &0.073 &0.006 &0.136 \\
MultiVAE &0.075 &0.012 &0.069 &0.007 &0.157 \\
BPRMF &0.032 &0.005 &0.027 &0.003 &0.076 \\
MostPop &0.019 &0.003 &0.018 &0.002 &0.046 \\
Random &0.001 &0.000 &0.001 &0.000 &0.004 \\
\bottomrule
\end{tabularx}
\end{table} 

==> tables/amazon_beyond.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Beyond Accuracy Results for Amazon Digital Music. The Tables are sorted by nDCG in descending order. The notation \emph{@N} indicates that the metrics are computed considering recommendation lists of \emph{N} elements.}\label{tab: }
\scriptsize
\begin{tabular}{lrrrrrrrrr}\toprule
\textbf{Algorithm} &\textbf{IC@10} &\textbf{Gini@10} &\textbf{EFD@10} &\textbf{EPC@10} &\textbf{PopREO@10} &\textbf{PopRSP@10} &\textbf{ACLT@10} &\textbf{APLT@10} &\textbf{ARP@10} \\\midrule
\pbeta &9959.000 &0.542 &0.409 &0.033 &0.308 &0.334 &2.986 &0.299 &23.759 \\
\slim &8215.400 &0.197 &0.361 &0.030 &0.552 &0.845 &0.668 &0.067 &49.287 \\
\userknn &7703.800 &0.181 &0.363 &0.030 &0.552 &0.870 &0.560 &0.056 &51.910 \\
\easer &7887.200 &0.170 &0.337 &0.029 &0.559 &0.869 &0.563 &0.056 &66.180 \\
\ials &4516.200 &0.136 &0.325 &0.027 &0.766 &0.980 &0.087 &0.009 &41.936 \\
\itemknn &9686.200 &0.478 &0.345 &0.027 &0.097 &0.179 &5.504 &0.550 &9.884 \\
MF2020 &4722.800 &0.099 &0.242 &0.021 &0.687 &0.979 &0.092 &0.009 &59.949 \\
NeuMF &7365.200 &0.228 &0.245 &0.020 &0.455 &0.865 &0.583 &0.058 &30.236 \\
MultiVAE &6043.000 &0.189 &0.235 &0.020 &0.578 &0.896 &0.448 &0.045 &40.475 \\
BPRMF &3050.000 &0.024 &0.078 &0.007 &0.784 &0.997 &0.013 &0.001 &130.810 \\
MostPop &15.600 &0.001 &0.039 &0.004 &1.000 &1.000 &0.000 &0.000 &182.800 \\
Random &10025.800 &0.852 &0.002 &0.000 &0.229 &0.002 &4.600 &0.460 &9.840 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrr}\toprule
\textbf{Algorithm} &\textbf{IC@20} &\textbf{Gini@20} &\textbf{EFD@20} &\textbf{EPC@20} &\textbf{PopREO@20} &\textbf{PopRSP@20} &\textbf{ACLT@20} &\textbf{APLT@20} &\textbf{ARP@20} \\\midrule
\pbeta &10016.000 &0.609 &0.293 &0.024 &0.318 &0.333 &5.978 &0.299 &22.353 \\
\slim &9659.400 &0.253 &0.263 &0.022 &0.548 &0.801 &1.719 &0.086 &43.337 \\
\userknn &9294.200 &0.237 &0.264 &0.022 &0.543 &0.832 &1.451 &0.073 &45.834 \\
\easer &9502.000 &0.224 &0.248 &0.021 &0.558 &0.829 &1.475 &0.074 &55.485 \\
\ials &5941.600 &0.177 &0.243 &0.020 &0.700 &0.964 &0.306 &0.015 &37.520 \\
\itemknn &9976.200 &0.528 &0.247 &0.019 &0.121 &0.171 &10.922 &0.546 &9.870 \\
MF2020 &6389.400 &0.135 &0.187 &0.016 &0.661 &0.966 &0.290 &0.014 &51.479 \\
NeuMF &8533.200 &0.266 &0.180 &0.015 &0.468 &0.827 &1.494 &0.075 &27.416 \\
MultiVAE &9161.400 &0.329 &0.178 &0.015 &0.519 &0.783 &1.881 &0.094 &33.590 \\
BPRMF &4283.000 &0.034 &0.064 &0.006 &0.787 &0.996 &0.034 &0.002 &108.296 \\
MostPop &29.200 &0.002 &0.033 &0.004 &1.000 &1.000 &0.000 &0.000 &148.838 \\
Random &10025.800 &0.895 &0.002 &0.000 &0.158 &0.002 &9.191 &0.460 &9.838 \\
\bottomrule
\end{tabular}


\begin{tabular}{lrrrrrrrrr}\toprule
\textbf{Algorithm} &\textbf{IC@50} &\textbf{Gini@50} &\textbf{EFD@50} &\textbf{EPC@50} &\textbf{PopREO@50} &\textbf{PopRSP@50} &\textbf{ACLT@50} &\textbf{APLT@50} &\textbf{ARP@50} \\\midrule
\pbeta &10018.600 &0.664 &0.182 &0.015 &0.330 &0.344 &14.694 &0.294 &20.677 \\
\slim &10009.200 &0.347 &0.165 &0.014 &0.528 &0.717 &6.159 &0.123 &35.188 \\
\userknn &9962.200 &0.329 &0.166 &0.014 &0.522 &0.760 &5.202 &0.104 &37.407 \\
\easer &10006.600 &0.318 &0.157 &0.013 &0.541 &0.746 &5.513 &0.110 &42.919 \\
\ials &8193.600 &0.253 &0.157 &0.013 &0.596 &0.914 &1.845 &0.037 &31.721 \\
\itemknn &10017.800 &0.586 &0.153 &0.012 &0.154 &0.110 &25.770 &0.515 &10.103 \\
MF2020 &8657.400 &0.201 &0.127 &0.011 &0.626 &0.930 &1.506 &0.030 &41.187 \\
NeuMF &9503.000 &0.327 &0.116 &0.009 &0.478 &0.756 &5.302 &0.106 &23.635 \\
MultiVAE &9806.600 &0.396 &0.119 &0.010 &0.514 &0.723 &6.034 &0.121 &29.196 \\
BPRMF &6450.600 &0.057 &0.046 &0.004 &0.801 &0.992 &0.168 &0.003 &82.728 \\
MostPop &64.400 &0.005 &0.025 &0.003 &1.000 &1.000 &0.000 &0.000 &113.346 \\
Random &10025.800 &0.933 &0.002 &0.000 &0.140 &0.001 &22.936 &0.459 &9.836 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/amazon_params.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[ht!]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\begin{tabular}{p{0.1\linewidth}p{0.15\linewidth}|wc{0.2\linewidth}}\toprule
Algorithm &Hyperparameter &Value \\\midrule
\multirow{2}{*}{UserKNN} &topK &226 \\
&similarity &cosine \\
\multirow{2}{*}{UserKNN} &topK &798 \\
&similarity &cosine \\
\multirow{4}{*}{RP3beta} &topK &803 \\
&alpha &0.4973207 \\
&beta &0.2836938 \\
&normalization &false \\
\multirow{3}{*}{SLIM} &topK &663 \\
&l1 ratio &0.0000108 \\
&alpha &0.0486771 \\
EASER &l2 norm &238.5621338 \\
\multirow{4}{*}{MF2020} &num factors &64 \\
&learning rate &0.1295965 \\
&reg &0.0125009 \\
&negative sample &8 \\
\multirow{6}{*}{iALS} &num factors &200 \\
&epochs &70 \\
&scaling &log \\
&alpha &9.1219718 \\
&epsilon &0.4921936 \\
&reg &0.4921936 \\
\multirow{7}{*}{BPRMF} &num factors &64 \\
&epochs &86 \\
&learning rate &0.1265624 \\
&batch size &256 \\
&reg user &0.0058673 \\
&reg positive item &0.0052985 \\
&reg negative item &0.0009577 \\
\multirow{5}{*}{NeuMF} &num factors &128 \\
&epochs &100 \\
&learning rate &0.0001365 \\
&batch size &64 \\
&negative sample &6 \\
\multirow{4}{*}{MultiVAE} &epochs &205 \\
&learning rate &0.0000723 \\
&batch\_size &128 \\
&reg &0.1153400 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/borda_count_all_tops.tex <==
\begin{table}[H]

\small
\rowcolors{2}{white}{gray!15}
\begin{tabular}{crc}\hline
  \textbf{Rank} & \textbf{Algorithm} & \textbf{Count} \\ \hline
1 & \easer & 552 \\
2 & \slim &  485 \\
3 & \pbeta &  484 \\
4 & \userknn &  443 \\
5 & MF2020 &  363  \\
6 & MultiVAE &  304  \\
7 & \ials &  280  \\
8 & \itemknn &  279  \\
9 & NeuMF &  184  \\
10 & BPRMF &  136  \\
11 & MostPop &  54  \\
12 & Random &  0  \\  \bottomrule
\end{tabular}
\caption{Overall}\label{subtab:borda-count}
\end{table}

==> tables/epinions_accuracy.tex <==
\begin{table}[H]
\centering
\caption{Accuracy Results for Epinions. The Tables are sorted by nDCG in descending order. The notation \emph{@N} indicates that the metrics are computed considering recommendation lists of \emph{N} elements.}
\label{tab:movielens_accuracy}
%\rowcolors{1}{white}{gray!15}
% \renewcommand{\arraystretch}{0.8}
% \rowcolors{2}{gray!15}{white}
% \begin{tabular}{lrrrrrrrrrrr}\hline
%     \multirow{2}{*}{\textbf{Algorithm}} &\multicolumn{5}{c}{\textbf{Top@10}}&\multicolumn{5}{c}{\textbf{Top@50}} \\
%     \cmidrule(lr){2-6} \cmidrule(l){7-11}
% &\textbf{nDCG} &\textbf{MAP} &\textbf{MRR} &\textbf{Pre} &\textbf{Rec}
% &\textbf{nDCG} &\textbf{MAP} &\textbf{MRR} &\textbf{Pre} &\textbf{Rec}\\\midrule


% MultiVAE &0.149 &0.116 &0.240 &0.148 &0.094 &0.202 &0.077 &0.269 &0.046 &0.305 \\
% NeuMF &0.118 &0.098 &0.206 &0.108 &0.080 &0.162 &0.064 &0.216 &0.043 &0.260 \\
% \pbeta &\underline{0.163} &\underline{0.129} &\underline{0.260} &\textbf{0.159} &\textbf{0.102} &\underline{0.202} &\underline{0.077} &0.269 &0.046 &0.305 \\
% \easer &0.096 &0.078 &0.176 &0.089 &0.060 &0.129 &0.048 &0.186 &0.032 &0.211 \\
% \slim &0.156 &0.126 &0.254 &0.148 &\underline{0.101} &\underline{0.202} &\textbf{0.078} &\underline{0.264} &\textbf{0.049} &\underline{0.314} \\
% \ials &0.110 &0.091 &0.192 &0.101 &0.074 &0.147 &0.058 &0.201 &0.037 &0.231 \\
% BPRMF  &0.113 &0.093 &0.200 &0.106 &0.076 &0.157 &0.061 &0.211 &0.041 &0.260 \\
% MF2020 &0.125 &0.104 &0.219 &0.114 &0.084 &0.171 &0.067 &0.229 &0.044 &0.279 \\
% \userknn &\textbf{0.164} &\textbf{0.131} &\textbf{0.266} &\underline{0.157} &\textbf{0.102} &\textbf{0.208} &\textbf{0.078} &\textbf{0.275} &\underline{0.048} &\textbf{0.318} \\
% \itemknn &0.138 &0.111 &0.224 &0.133 &0.090 &0.179 &0.069 &0.233 &0.044 &0.282 \\
% MostPop &0.045 &0.037 &0.093 &0.036 &0.029 &0.067 &0.026 &0.103 &0.019 &0.111 \\
% Random &0.001 &0.001 &0.003 &0.001 &0.001 &0.003 &0.001 &0.004 &0.001 &0.006 \\
% \bottomrule
% \end{tabular}


\scriptsize
\begin{tabularx}{0.48\textwidth}{Xrrrrrr}\toprule
\textbf{Algorithm} &\textbf{nDCG@10} &\textbf{MAP@10} &\textbf{MRR@10} &\textbf{Pre@10} &\textbf{Rec@10} \\\midrule
\userknn &0.164 &0.131 &0.266 &0.102 &0.157 \\
\pbeta &0.163 &0.129 &0.260 &0.102 &0.159 \\
\slim &0.156 &0.126 &0.254 &0.101 &0.148 \\
MultiVAE &0.149 &0.116 &0.240 &0.094 &0.148 \\
\itemknn &0.138 &0.111 &0.224 &0.090 &0.133 \\
MF2020 &0.125 &0.104 &0.219 &0.084 &0.114 \\
NeuMF &0.118 &0.098 &0.206 &0.080 &0.108 \\
BPRMF &0.113 &0.093 &0.200 &0.076 &0.106 \\
\ials &0.110 &0.091 &0.192 &0.074 &0.101 \\
\easer &0.096 &0.078 &0.176 &0.060 &0.089 \\
MostPop &0.045 &0.037 &0.093 &0.029 &0.036 \\
Random &0.001 &0.001 &0.003 &0.001 &0.001 \\
\bottomrule
\end{tabularx}

% \rowcolors{1}{white}{gray!15}
\begin{tabularx}{0.48\textwidth}{Xrrrrrr}\toprule
\textbf{Algorithm} &\textbf{nDCG@20} &\textbf{MAP@20} &\textbf{MRR@20} &\textbf{Pre@20} &\textbf{Rec@20} \\\midrule
\userknn &0.178 &0.108 &0.272 &0.076 &0.219 \\
\pbeta &0.176 &0.107 &0.266 &0.075 &0.218 \\
\slim &0.170 &0.106 &0.260 &0.076 &0.210 \\
MultiVAE &0.165 &0.099 &0.247 &0.072 &0.212 \\
\itemknn &0.151 &0.094 &0.230 &0.068 &0.190 \\
MF2020 &0.138 &0.088 &0.225 &0.065 &0.170 \\
NeuMF &0.131 &0.084 &0.212 &0.063 &0.162 \\
BPRMF &0.126 &0.079 &0.207 &0.060 &0.160 \\
\ials &0.121 &0.077 &0.198 &0.057 &0.149 \\
\easer &0.105 &0.065 &0.182 &0.046 &0.130 \\
MostPop &0.052 &0.032 &0.100 &0.025 &0.061 \\
Random &0.002 &0.001 &0.003 &0.001 &0.002 \\
\bottomrule
\end{tabularx}

% \rowcolors{1}{white}{gray!15}
\begin{tabularx}{0.48\textwidth}{Xrrrrrr}\toprule
\textbf{Algorithm} &\textbf{nDCG@50} &\textbf{MAP@50} &\textbf{MRR@50} &\textbf{Pre@50} &\textbf{Rec@50} \\\midrule
\userknn &0.208 &0.078 &0.275 &0.048 &0.318 \\
\slim &0.202 &0.078 &0.264 &0.049 &0.314 \\
\pbeta &0.202 &0.077 &0.269 &0.046 &0.305 \\
MultiVAE &0.198 &0.073 &0.251 &0.047 &0.317 \\
\itemknn &0.179 &0.069 &0.233 &0.044 &0.282 \\
MF2020 &0.171 &0.067 &0.229 &0.044 &0.279 \\
NeuMF &0.162 &0.064 &0.216 &0.043 &0.260 \\
BPRMF &0.157 &0.061 &0.211 &0.041 &0.260 \\
\ials &0.147 &0.058 &0.201 &0.037 &0.231 \\
\easer &0.129 &0.048 &0.186 &0.032 &0.211 \\
MostPop &0.067 &0.026 &0.103 &0.019 &0.111 \\
Random &0.003 &0.001 &0.004 &0.001 &0.006 \\
\bottomrule
\end{tabularx}
\end{table} 

==> tables/epinions_beyond.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Beyond Accuracy Results for Epinions. The Tables are sorted by nDCG in descending order. The notation \emph{@N} indicates that the metrics are computed considering recommendation lists of \emph{N} elements. \textcolor{blue}{To ease the interpretation of the results and associate higher values to diversified recommendation lists, we report the value of 1-Gini.}}\label{tab: }
\scriptsize
\begin{tabular}{lrrrrrrrrr}\toprule
\textbf{Algorithm} &\textbf{IC@10} &\textbf{Gini@10} &\textbf{EFD@10} &\textbf{EPC@10} &\textbf{PopREO@10} &\textbf{PopRSP@10} &\textbf{ACLT@10} &\textbf{APLT@10} &\textbf{ARP@10} \\\midrule
\userknn &3402.200 &0.073 &1.198 &0.112 &0.398 &0.940 &0.803 &0.080 &315.724 \\
\pbeta &6009.000 &0.197 &1.237 &0.112 &0.198 &0.763 &2.746 &0.275 &226.165 \\
\slim &3361.000 &0.081 &1.197 &0.110 &0.452 &0.955 &0.613 &0.061 &246.216 \\
MultiVAE &3386.800 &0.089 &1.105 &0.102 &0.364 &0.920 &1.048 &0.105 &293.641 \\
\itemknn &5832.800 &0.160 &1.084 &0.097 &0.171 &0.771 &2.670 &0.267 &214.681 \\
MF2020 &1235.200 &0.028 &0.921 &0.090 &0.786 &0.994 &0.081 &0.008 &368.003 \\
NeuMF &3595.000 &0.084 &0.905 &0.085 &0.495 &0.927 &0.960 &0.096 &322.865 \\
BPRMF &1322.800 &0.018 &0.824 &0.081 &0.651 &0.991 &0.121 &0.012 &475.629 \\
\ials &1613.400 &0.064 &0.891 &0.081 &0.707 &0.993 &0.104 &0.010 &214.989 \\
\easer &1598.200 &0.010 &0.633 &0.065 &0.683 &0.987 &0.177 &0.018 &577.325 \\
MostPop &41.600 &0.001 &0.273 &0.030 &1.000 &1.000 &0.000 &0.000 &719.301 \\
Random &8443.000 &0.823 &0.011 &0.001 &0.142 &0.003 &7.385 &0.738 &27.565 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrr}\toprule
\textbf{Algorithm} &\textbf{IC@20} &\textbf{Gini@20} &\textbf{EFD@20} &\textbf{EPC@20} &\textbf{PopREO@20} &\textbf{PopRSP@20} &\textbf{ACLT@20} &\textbf{APLT@20} &\textbf{ARP@20} \\\midrule
\userknn &4594.6 &0.09517 &0.96207 &0.08977 &0.44219 &0.93753 &1.66734 &0.08337 &275.26501 \\
\pbeta &7010.8 &0.23180 &0.98292 &0.08889 &0.26189 &0.77035 &5.35807 &0.26790 &198.23989 \\
\slim &4401.2 &0.09787 &0.96461 &0.08902 &0.49320 &0.95376 &1.25179 &0.06259 &228.15516 \\
MultiVAE &4249.6 &0.11247 &0.90021 &0.08286 &0.42643 &0.91431 &2.24238 &0.11212 &255.45705 \\
\itemknn &7100.2 &0.18764 &0.87540 &0.07898 &0.27226 &0.77605 &5.24759 &0.26238 &199.48788 \\
MF2020 &1631.2 &0.03964 &0.76576 &0.07432 &0.77640 &0.99373 &0.17579 &0.00879 &320.86731 \\
NeuMF &4647.0 &0.10828 &0.75634 &0.07108 &0.54241 &0.91979 &2.10595 &0.10530 &276.81741 \\
BPRMF &1793.6 &0.02597 &0.69284 &0.06708 &0.64018 &0.99133 &0.24262 &0.01213 &409.83159 \\
\ials &2052.0 &0.07826 &0.73017 &0.06620 &0.65387 &0.98884 &0.31170 &0.01559 &202.71822 \\
\easer &2509.6 &0.01487 &0.51832 &0.05260 &0.71106 &0.98731 &0.35378 &0.01769 &507.40035 \\
MostPop &72.0 &0.00248 &0.24410 &0.02655 &1.00000 &1.00000 &0.00000 &0.00000 &629.74485 \\
Random &8443.6 &0.87457 &0.01062 &0.00090 &0.07852 &0.00062 &14.75045 &0.73752 &27.65366 \\
\bottomrule
\end{tabular}


\begin{tabular}{lrrrrrrrrr}\toprule
\textbf{Algorithm} &\textbf{IC@50} &\textbf{Gini@50} &\textbf{EFD@50} &\textbf{EPC@50} &\textbf{PopREO@50} &\textbf{PopRSP@50} &\textbf{ACLT@50} &\textbf{APLT@50} &\textbf{ARP@50} \\\midrule
\userknn &6462.200 &0.136 &0.667 &0.062 &0.496 &0.928 &4.781 &0.096 &225.490 \\
\slim &6133.000 &0.129 &0.675 &0.062 &0.542 &0.947 &3.557 &0.071 &199.223 \\
\pbeta &7908.400 &0.287 &0.668 &0.060 &0.341 &0.764 &13.685 &0.274 &162.134 \\
MultiVAE &5567.600 &0.152 &0.637 &0.059 &0.491 &0.902 &6.368 &0.127 &211.471 \\
\itemknn &8192.000 &0.232 &0.611 &0.055 &0.379 &0.774 &13.230 &0.265 &177.703 \\
MF2020 &2286.000 &0.062 &0.564 &0.054 &0.766 &0.991 &0.630 &0.013 &263.954 \\
NeuMF &6027.600 &0.149 &0.554 &0.052 &0.586 &0.905 &6.186 &0.124 &224.754 \\
BPRMF &2533.400 &0.042 &0.512 &0.049 &0.653 &0.991 &0.596 &0.012 &331.178 \\
\ials &2826.800 &0.103 &0.517 &0.047 &0.617 &0.982 &1.276 &0.026 &183.072 \\
\easer &4381.600 &0.026 &0.383 &0.038 &0.746 &0.987 &0.931 &0.019 &412.526 \\
MostPop &151.000 &0.006 &0.197 &0.021 &1.000 &1.000 &0.000 &0.000 &506.930 \\
Random &8443.600 &0.921 &0.010 &0.001 &0.047 &0.001 &36.801 &0.736 &27.645 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/epinions_params.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[ht!]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\begin{tabular}{p{0.1\linewidth}p{0.15\linewidth}|wc{0.2\linewidth}}\toprule
Algorithm &Hyperparameter &Value \\\midrule
\multirow{2}{*}{UserKNN} &topK &139 \\
&similarity &cosine \\
\multirow{2}{*}{ItemNN} &topK &137 \\
&similarity &cosine \\
\multirow{4}{*}{RP3beta} &topK &144 \\
&alpha &0.8719344 \\
&beta &0.2483698 \\
&normalization &true \\
\multirow{3}{*}{SLIM} &topK &663 \\
&l1 ratio &0.0000108 \\
&alpha &0.0486771 \\
EASER &l2 norm &238.5621338 \\
\multirow{5}{*}{MF2020} &num factors &16 \\
&epochs &97 \\
&learning rate &0.0154435 \\
&reg &0.0223642 \\
&negative sample &4 \\
\multirow{6}{*}{iALS} &num factors &178 \\
&epochs &145 \\
&scaling &log \\
&alpha &2.8537184 \\
&epsilon &2.3098481 \\
&reg &0.0411491 \\
\multirow{7}{*}{BPRMF} &num factors &256 \\
&epochs &63 \\
&learning rate &0.1004075 \\
&batch size &256 \\
&reg user &0.0002613 \\
&reg positive item &0.0034511 \\
&reg negative item &0.0328127 \\
\multirow{5}{*}{NeuMF} &num factors &32 \\
&epochs &39 \\
&learning rate &0.0000465 \\
&batch size &256 \\
&negative sample &8 \\
\multirow{6}{*}{MultiVAE} &epochs &200 \\
&learning rate &0.0001003 \\
&batch\_size &128 \\
&intermediate dim &674 \\
&latent dim &175 \\
&reg &0.0020018 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/ml1m_accuracy.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[H]
\centering
\caption{Accuracy Results for MovieLens-1M. The Tables are sorted by nDCG in descending order. The notation \emph{@N} indicates that the metrics are computed considering recommendation lists of \emph{N} elements.}
\label{tab:movielens_accuracy}
%\rowcolors{1}{white}{gray!15}
% \renewcommand{\arraystretch}{0.8}
% \rowcolors{2}{gray!15}{white}
% \begin{tabular}{lrrrrrrrrrrr}\hline
%     \multirow{2}{*}{\textbf{Algorithm}} &\multicolumn{5}{c}{\textbf{Top@10}}&\multicolumn{5}{c}{\textbf{Top@50}} \\
%     \cmidrule(lr){2-6} \cmidrule(l){7-11}
% &\textbf{nDCG} &\textbf{MAP} &\textbf{MRR} &\textbf{Pre} &\textbf{Rec}
% &\textbf{nDCG} &\textbf{MAP} &\textbf{MRR} &\textbf{Pre} &\textbf{Rec}\\\midrule
% MultiVAE &0.294 &0.284 &0.514 &0.243 &0.183 &0.352 &0.198 &0.520 &0.139 &\underline{0.448} \\
% NeuMF &0.277 &0.275 &0.494 &0.232 &0.157 &0.322 &0.189 &0.502 &0.132 &0.406 \\
% \pbeta &0.315 &0.313 &0.556 &0.256 &0.184 &0.355 &\underline{0.206} &0.562 &0.138 &0.434 \\
% \easer &0.202 &0.205 &0.404 &0.166 &0.107 &0.226 &0.134 &0.415 &0.094 &0.277 \\
%\\slim &\textbf{0.335} &\textbf{0.337} &\textbf{0.580} &\textbf{0.275} &\underline{0.189} &\underline{0.368} &\textbf{0.218} &\textbf{0.586} &\underline{0.144} &0.440 \\
% \ials &0.306 &0.304 &0.542 &0.252 &0.179 &0.351 &0.204 &0.548 &0.139 &0.431 \\
% BPRMF &0.275 &0.271 &0.502 &0.226 &0.166 &0.324 &0.183 &0.510 &0.126 &0.409 \\
% MF2020 &\underline{0.329} &\underline{0.327} &\underline{0.563} &\underline{0.272} &\textbf{0.190} &\textbf{0.371} &\textbf{0.218} &\underline{0.569} &\textbf{0.148} &\textbf{0.454} \\
% \userknn &0.315 &0.314 &0.554 &0.256 &0.183 &0.351 &0.204 &0.561 &0.136 &0.426 \\
% \itemknn &0.292 &0.293 &0.518 &0.242 &0.163 &0.326 &0.194 &0.525 &0.131 &0.397 \\
% MostPop &0.159 &0.159 &0.317 &0.137 &0.084 &0.185 &0.113 &0.330 &0.081 &0.237 \\
% Random &0.008 &0.007 &0.020 &0.007 &0.004 &0.013 &0.007 &0.028 &0.007 &0.019 \\
% \bottomrule
% \end{tabular}

\scriptsize
\begin{tabularx}{\textwidth}{Xrrrrrr}\toprule
\textbf{Algorithm} &\textbf{nDCG@10} &\textbf{MAP@10} &\textbf{MRR@10} &\textbf{Pre@10} &\textbf{Rec@10} \\\midrule
\slim &0.335 &0.337 &0.580 &0.275 &0.189  \\
MF2020 &0.329 &0.327 &0.563 &0.272 &0.190 \\
\userknn &0.315 &0.314 &0.554 &0.256 &0.183 \\
\pbeta &0.315 &0.313 &0.556 &0.256 &0.184\\
\ials &0.306 &0.304 &0.542 &0.252 &0.179  \\
MultiVAE &0.294 &0.284 &0.514 &0.243 &0.183 \\
\itemknn &0.292 &0.293 &0.518 &0.242 &0.163 \\
NeuMF &0.277 &0.275 &0.494 &0.232 &0.157\\
BPRMF &0.275 &0.271 &0.502 &0.226 &0.166 \\
\easer &0.202 &0.205 &0.404 &0.166 &0.107 \\
MostPop &0.159 &0.159 &0.317 &0.137 &0.084 \\
Random &0.008 &0.007 &0.020 &0.007 &0.004\\
\bottomrule
\end{tabularx}


%\rowcolors{1}{white}{gray!15}
\begin{tabularx}{\textwidth}{Xrrrrrr}\toprule
\textbf{Algorithm} &\textbf{nDCG@20} &\textbf{MAP@20} &\textbf{MRR@20} &\textbf{Pre@20} &\textbf{Rec@20} \\\midrule
\slim &0.332 &0.288 &0.584 &0.216 &0.283 \\
MF2020 &0.329 &0.283 &0.568 &0.216 &0.286 \\
\pbeta &0.315 &0.269 &0.561 &0.203 &0.277 \\
\userknn &0.314 &0.268 &0.559 &0.201 &0.273 \\
\ials &0.309 &0.263 &0.547 &0.202 &0.272 \\
MultiVAE &0.304 &0.250 &0.519 &0.199 &0.281 \\
\itemknn &0.289 &0.252 &0.523 &0.192 &0.247 \\
BPRMF &0.280 &0.235 &0.508 &0.181 &0.253 \\
NeuMF &0.280 &0.240 &0.500 &0.188 &0.245 \\
\easer &0.197 &0.175 &0.412 &0.131 &0.163 \\
MostPop &0.161 &0.141 &0.326 &0.114 &0.137 \\
Random &0.009 &0.007 &0.024 &0.007 &0.007 \\
\bottomrule
\end{tabularx}

% \rowcolors{1}{white}{gray!15}
\begin{tabularx}{\textwidth}{Xrrrrrr}\toprule
\textbf{Algorithm} &\textbf{nDCG@50} &\textbf{MAP@50} &\textbf{MRR@50} &\textbf{Pre@50} &\textbf{Rec@50} \\\midrule
MF2020 &0.371 &0.218 &0.569 &0.148 &0.454 \\
\slim &0.368 &0.218 &0.586 &0.144 &0.440 \\
\pbeta &0.355 &0.206 &0.562 &0.138 &0.434 \\
MultiVAE &0.352 &0.198 &0.520 &0.139 &0.448 \\
\userknn &0.351 &0.204 &0.561 &0.136 &0.426 \\
\ials &0.351 &0.204 &0.548 &0.139 &0.431 \\
\itemknn &0.326 &0.194 &0.525 &0.131 &0.397 \\
BPRMF  &0.324 &0.183 &0.510 &0.126 &0.409 \\
NeuMF &0.322 &0.189 &0.502 &0.132 &0.406 \\
\easer &0.226 &0.134 &0.415 &0.094 &0.277 \\
MostPop &0.185 &0.113 &0.330 &0.081 &0.237 \\
Random &0.013 &0.007 &0.028 &0.007 &0.019 \\
\bottomrule
\end{tabularx}
\end{table} 

==> tables/ml1m_beyond.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Beyond Accuracy Results for MovieLens-1M. The Tables are sorted by nDCG in descending order. The notation \emph{@N} indicates that the metrics are computed considering recommendation lists of \emph{N} elements.}\label{tab: }
\scriptsize
\begin{tabular}{lrrrrrrrrr}\toprule
\textbf{Algorithm} &\textbf{IC@10} &\textbf{Gini@10} &\textbf{EFD@10} &\textbf{EPC@10} &\textbf{PopREO@10} &\textbf{PopRSP@10} &\textbf{ACLT@10} &\textbf{APLT@10} &\textbf{ARP@10} \\\midrule
\slim &654.200 &0.052 &2.672 &0.244 &0.995 &0.999 &0.009 &0.001 &1,121.384 \\
MF2020 &920.200 &0.077 &2.672 &0.244 &0.968 &0.995 &0.053 &0.005 &1,042.373 \\
\userknn &1,075.200 &0.067 &2.489 &0.227 &0.971 &0.992 &0.096 &0.010 &1,085.550 \\
\pbeta &854.400 &0.048 &2.461 &0.223 &0.959 &0.990 &0.114 &0.011 &1,181.638 \\
\ials &712.200 &0.080 &2.516 &0.232 &0.997 &1.000 &0.004 &0.000 &935.914 \\
MultiVAE &1,625.200 &0.136 &2.422 &0.221 &0.828 &0.962 &0.423 &0.042 &871.869 \\
\itemknn &1,054.800 &0.066 &2.346 &0.214 &0.952 &0.990 &0.112 &0.011 &1,090.926 \\
NeuMF &1,367.200 &0.111 &2.292 &0.209 &0.910 &0.975 &0.282 &0.028 &938.861 \\
BPRMF &1,137.800 &0.091 &2.226 &0.203 &0.928 &0.991 &0.105 &0.010 &1,047.232 \\
\easer &64.400 &0.006 &1.506 &0.132 &1.000 &1.000 &0.000 &0.000 &1,709.339 \\
MostPop &56.200 &0.005 &1.187 &0.103 &1.000 &1.000 &0.000 &0.000 &1,746.694 \\
Random &2,810.000 &0.876 &0.074 &0.006 &0.039 &0.005 &6.958 &0.696 &151.045 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrrrrrrr}\toprule
\textbf{Algorithm} &\textbf{IC@20} &\textbf{Gini@20} &\textbf{EFD@20} &\textbf{EPC@20} &\textbf{PopREO@20} &\textbf{PopRSP@20} &\textbf{ACLT@20} &\textbf{APLT@20} &\textbf{ARP@20} \\\midrule
\slim &854.000 &0.069 &2.239 &0.205 &0.986 &0.998 &0.050 &0.003 &1017.374 \\
MF2020 &1128.800 &0.095 &2.257 &0.207 &0.946 &0.992 &0.184 &0.009 &969.260 \\
\pbeta &1207.200 &0.073 &2.085 &0.190 &0.937 &0.984 &0.359 &0.018 &1024.408 \\
\userknn &1465.800 &0.092 &2.090 &0.191 &0.947 &0.985 &0.333 &0.017 &970.255 \\
\ials &901.000 &0.105 &2.138 &0.197 &0.983 &0.998 &0.040 &0.002 &838.660 \\
MultiVAE &1924.800 &0.156 &2.082 &0.190 &0.792 &0.953 &1.042 &0.052 &821.849 \\
\itemknn &1346.000 &0.082 &1.977 &0.181 &0.939 &0.987 &0.297 &0.015 &1006.978 \\
BPRMF &1386.200 &0.111 &1.893 &0.173 &0.890 &0.985 &0.343 &0.017 &968.784 \\
NeuMF &1679.400 &0.135 &1.965 &0.179 &0.867 &0.966 &0.762 &0.038 &868.452 \\
\easer &115.200 &0.011 &1.265 &0.113 &1.000 &1.000 &0.000 &0.000 &1542.211 \\
MostPop &92.000 &0.010 &1.039 &0.092 &1.000 &1.000 &0.000 &0.000 &1570.672 \\
Random &2810.000 &0.911 &0.075 &0.007 &0.037 &0.002 &13.867 &0.693 &151.352 \\
\bottomrule
\end{tabular}


\begin{tabular}{lrrrrrrrrr}\toprule
\textbf{Algorithm} &\textbf{IC@50} &\textbf{Gini@50} &\textbf{EFD@50} &\textbf{EPC@50} &\textbf{PopREO@50} &\textbf{PopRSP@50} &\textbf{ACLT@50} &\textbf{APLT@50} &\textbf{ARP@50} \\\midrule
MF2020 &1434.200 &0.129 &1.683 &0.154 &0.881 &0.982 &1.020 &0.020 &845.432 \\
\slim &1183.200 &0.104 &1.645 &0.151 &0.961 &0.994 &0.347 &0.007 &865.957 \\
\pbeta &1739.400 &0.124 &1.556 &0.142 &0.878 &0.965 &1.923 &0.038 &818.995 \\
MultiVAE &2310.200 &0.195 &1.576 &0.144 &0.711 &0.932 &3.699 &0.074 &730.213 \\
\userknn &2096.400 &0.141 &1.548 &0.142 &0.887 &0.967 &1.844 &0.037 &816.321 \\
\ials &1241.200 &0.153 &1.601 &0.147 &0.917 &0.989 &0.648 &0.013 &703.357 \\
\itemknn &1792.800 &0.112 &1.472 &0.135 &0.913 &0.981 &1.043 &0.021 &872.677 \\
BPRMF &1728.400 &0.151 &1.430 &0.130 &0.785 &0.969 &1.745 &0.035 &831.305 \\
NeuMF &2122.200 &0.180 &1.494 &0.136 &0.776 &0.945 &3.022 &0.060 &754.619 \\
\easer &222.800 &0.026 &0.975 &0.088 &1.000 &1.000 &0.000 &0.000 &1236.443 \\
MostPop &188.200 &0.023 &0.809 &0.073 &1.000 &1.000 &0.000 &0.000 &1256.676 \\
Random &2810.000 &0.941 &0.077 &0.007 &0.026 &0.001 &34.450 &0.689 &151.523 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/ml1m_params.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[ht!]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\begin{tabular}{p{0.1\linewidth}p{0.15\linewidth}|wc{0.2\linewidth}}\toprule
Algorithm &Hyperparameter &Value \\\midrule
\multirow{2}{*}{UserKNN} &topK &117 \\
&similarity &correlation \\\hline
\multirow{2}{*}{ItemKNN} &topK &95 \\
&similarity &cosine \\\hline
\multirow{4}{*}{RP3beta} &topK &158 \\
&alpha &1.4350197 \\
&beta &0.3265517 \\
&normalization &true \\\hline
\multirow{3}{*}{SLIM} &topK &518 \\
&l1 ratio &0.0000420 \\
&alpha &0.2978543 \\\hline
EASER &l2 norm &238.5621338 \\\hline
\multirow{5}{*}{MF2020} &num factors &128 \\
&epochs &72 \\
&learning rate &0.1295965 \\
reg &0.0087583 \\
&negative sample &4 \\\hline
\multirow{6}{*}{iALS} &num factors &51 \\
&epochs &27 \\
&scaling &log \\
&alpha &6.3818930 \\
&epsilon &5.6496278 \\
&reg &0.0494734 \\\hline
\multirow{7}{*}{BPRMF} &num factors &256 \\
&epochs &73 \\
&learning rate &0.0378936 \\
&batch size &256 \\
&reg user &0.0157839 \\
&reg positive item &0.0005651 \\
&reg negative item &0.0012779 \\\hline
\multirow{5}{*}{NeuMF} &num factors &16 \\
&epochs &93 \\
&learning rate &0.0000366 \\
&batch size &256 \\
&negative sample &6 \\\hline
\multirow{4}{*}{MultiVAE} &epochs &100 \\
&learning rate &0.0001545 \\
&batch\_size &128 \\
&reg &0.0000105 \\
\bottomrule
\end{tabular}
\end{table}
